Constraints on the End of Reionization from the Density Fields Surrounding Two Highly Opaque Quasar Sightlines

The observed large-scale scatter in Lyman $\alpha$ opacity of the intergalactic medium at $z<6$ implies large fluctuations in the neutral hydrogen fraction that are unexpected long after reionization has ended. A number of models have emerged to explain these fluctuations that make testable predictions for the relationship between Ly$\alpha$ opacity and density. We present selections of $z=5.7$ Ly$\alpha$-emitting galaxies (LAEs) in the fields surrounding two highly opaque quasar sightlines with long Ly$\alpha$ troughs. The fields lie towards the $z=6.0$ quasar ULAS J0148+0600, for which we re-analyze previously published results using improved photometric selection, and towards the $z=6.15$ quasar SDSS J1250+3130, for which results are presented here for the first time. In both fields, we report a deficit of LAEs within 20 $h^{-1}$ Mpc of the quasar. The association of highly opaque sightlines with galaxy underdensities in these two fields is consistent with models in which the scatter in Ly$\alpha$ opacity is driven by large-scale fluctuations in the ionizing UV background, or by an ultra-late reionization that has not yet concluded at $z=5.7$.

==> det_summary.tex <==

%\clearpage
\LongTables
\begin{center}
\begin{deluxetable}{ccc}
\tablewidth{0pc}
\tablecaption{Summary of Keck/DEIMOS followup of LAE candidates \label{tab:det_summary}}
\tabletypesize{\scriptsize}
\tablehead{\colhead{} & \colhead{This work}$^a$ & \colhead{\citet{becker18}} \\}
\startdata
LAE candidates$^a$ & 12 & 46 \\
Spectroscopically confirmed LAEs & 10 & 19 \\
Contaminants & 0 & 3 \\
Non-detections$^b$ 2 X & 24\\


\enddata
\tablenotetext{a}{LAE candidates for followup were selected from the ~\citet{becker18} catalog; not all of those candidates are selected in this work.}
\tablenotetext{b}{We attribute the large number of non-detections to the artificially high narrowband flux and S/N ratios reported for some objects in ~\citet{becker18}; all of the objects reported as non-detections were not selected as credible LAE candidates in this work, largely because they are too faint, don't meet the S/N ratio threshold, or both.}

\end{deluxetable}
\end{center}


%\multirow{3}{*}{J0148}

==> non_detections.tex <==

%\clearpage
\LongTables
\begin{center}
\begin{deluxetable*}{ccccccc}
\tablewidth{0pc}
\tablecaption{Summary of non-detected LAE candidates in the J0148 field}
\tabletypesize{\scriptsize}
\tablehead{\colhead{ID} & \colhead{RA (J200)} & \colhead{Dec (J1200)} & \colhead{m$_{\rm{NB816}}^a$}  & \colhead{ $F_{phot}$ ( $10^{-17}$ergs $s^{-1}$ cm$^{-2}$  )} & \colhead{ $F_{spec}$ (upper limit, $\cdot10^{-17}$ergs $s^{-1}$ cm$^{-2}$  )} & \colhead{Selected?}}
\startdata
J014838+060503&01h48m38.209s&+06d05m03.96s&26.38 & 1.38 $\pm$ 0.49&6.973 & N\\ 
J014856+060242&01h48m56.211s&+06d02m42.32s&25.77 & 2.4 $\pm$ 0.47&9.678 & N\\ 
J014842+055805&01h48m42.020s&+05d58m05.18s&25.4 & 3.39 $\pm$ 0.48&1.418 & N\\ 
J014916+055903&01h49m16.873s&+05d59m03.00s&25.81 & 2.31 $\pm$ 0.5&2.062 & N\\ 
J014842+055118&01h48m42.989s&+05d51m18.32s&26.03 & 1.9 $\pm$ 0.58&9.344 & N\\ 
J014844+055105&01h48m44.908s&+05d51m05.01s&26.61 & 1.11 $\pm$ 0.57&4.622 & N\\ 
J014855+055002&01h48m55.052&+05d50m02.93s&25.72 & 2.52 $\pm$ 0.64&4.486 & N\\ 
J014902+055034&01h49m02.475&+05d50m34.51s&26.02 & 1.9 $\pm$ 0.56&3.859 & N\\ 
J014918+054839&01h49m18.231s&+05d48m39.43s& X & X &4.23 & N\\ %not tagged as a source - do ap by hand
J014921+054808&01h49m21.717s&+05d48m08.95s&X & X&4.618 & N\\ %not tagged as a source - do ap by hand
J014926+054822&01h49m26.775s&+05d48m22.53s&25.51 & 3.05 $\pm$ 0.6&4.422 & N\\ 
J014931+054531&01h49m31.263s&+05d45m31.09s&26.61 & 1.11 $\pm$ 0.75&3.619 & N\\ 
J014937+054807&01h49m37.805s&+05d48m07.86s&25.54 & 2.98 $\pm$ 0.51&20.189 & Y\\ 
J014630+060502&01h46m30.381s&+06d05m02.51s&26.26 & 1.53 $\pm$ 0.48&3.366 & N\\ 
J014631+060139&01h46m31.089s&+06d01m39.76s&26.24 & 1.56 $\pm$ 0.58&3.411 & N\\
J014637+050210&01h46m37.775s&+06d02m10.95s&26.63 & 1.09 $\pm$ 0.58&3.054 & N\\
J014637+060130&01h46m37.460s&+06d01m30.73s&25.25 & 3.9 $\pm$ 0.51&3.369 & N\\ 
J014704+055642&01h47m04.90s&+05d56m42.81s&25.66 & 2.67 $\pm$ 0.63&3.176 & N\\ 
J014642+055310&01h46m42.847s&+05d53m10.51s&26.75 & 0.97 $\pm$ 0.49&2.696 & N\\ 
J014639+054905&01h46m39.634&+05d49m05.78s&25.15 & 4.26 $\pm$ 0.53&2.218 & Y\\ 
J014658+053843&01h46m58.197s&+05d38m43.73s&25.7 & 2.58 $\pm$ 0.68&2.374 & N\\ 
J014658+053744&01h46m58.182s&+05d37m44.67s&27.51 & 0.49 $\pm$ 0.85&2.177 & N\\ 


\enddata
\tablenotetext{a}{Photometric measurement}
\end{deluxetable*}
\end{center}


==> num_dens_j1250_v19.tex <==

%\clearpage
\LongTables
\begin{deluxetable}{lccc}
%\tablewidth{0.45\textwidth}
\tablewidth{0pc}
\tablecaption{LAE Number Density in the J1250 Field \label{tab:num_dens_j1250}}
\tabletypesize{\scriptsize}
\tablehead{\colhead{R (Mpc)}  & \colhead{$N_{LAEs}$} & \colhead{$N_{corr}^a$} & \colhead{$\Sigma$ LAE (Mpc h$^{-1}$)$^2$}}
\startdata
$5 (0-10)$  & 4 & 5 & 0.017 ($0.009-0.025$) \\
$15 (15-25)$  & 13 & 20 & 0.021 ($0.017-0.027$) \\
$25 (20-30)$  & 32 & 51 & 0.033 ($0.028-0.037$)\\
$35 (30-40)$  & 60 & 98 & 0.044 ($0.040-0.049$) \\
$45 (40-50)$  & 72 & 124 & 0.044 ($0.040-0.048$) \\
$55 (50-60)$  & 95 & 144 & 0.045 ($0.041-0.048$)\\
$65 (60-70)$  & 101 & 200 & 0.049 ($0.046-0.052$) \\
$72 (70-74.5)$  & 41 & 109 & 0.053 ($0.048-0.058$)
\enddata
\tablenotetext{a}{Completeness corrected}
\end{deluxetable}


==> table_template.tex <==

%\clearpage
\LongTables
\begin{center}
\begin{deluxetable}{llccc}
\tablewidth{0pc}
\tablecaption{Previous and Current Emission-Line Measurements of my DLA \label{tab:previous}}
\tabletypesize{\scriptsize}
\tablehead{\colhead{Line} & \colhead{Flux } & \colhead{FWHM} & \colhead{Redshift} & \colhead{Reference}\\
 & \colhead{[ergs s$^{-1}$ cm$^{-2}$] } & \colhead{[km s$^{-1}$]} &  }\\
\startdata
\lya & (6.4 $\pm$ 1.2)$\times$10$^{-17}$ & 200 & 3.1530 & a  \\

\enddata
\tablenotetext{f}{Unresolved line}
\end{deluxetable}
\end{center}

